Motives for Delegating Financial Decisions

Why do some investors delegate financial decisions to supposed experts? We report a laboratory experiment designed to disentangle four possible motives. Almost 600 investors drawn from the Prolific subject pool choose whether or not to delegate a real-stakes choice among lotteries to a previous investor (an ``expert'') after seeing information on the performance of several available experts. We find that a surprisingly large fraction of investors delegate even trivial choice tasks, suggesting a major role for the blame shifting motive. A larger fraction of investors delegate our more complex tasks, suggesting that decision costs play a role for some investors. Some investors who delegate choose a low quality expert with high earnings, suggesting a role for chasing past performance. We find no evidence for a fourth possible motive, that delegation makes risk more acceptable.

==> paper_Figs_and_Tabs/budgets.tex <==
\begin{figure}[htbp]
    \centering
\begin{subfigure}[t]{0.19\linewidth}
         \centering
\resizebox{1\linewidth}{!}{
    \begin{tikzpicture} \begin{axis}[
  xmin=-1, xmax=101,
  ymin=-1, ymax=101,
]  \addplot+[
  only marks,
  mark = square*,
  fill=blue,
  color=blue,
  mark size=2.9pt
  ]
  coordinates{
  (100,0)
  (0,100)};
  \end{axis}
  \end{tikzpicture}
}
\end{subfigure}   
\hfill
\begin{subfigure}[t]{0.19\linewidth}
         \centering
\resizebox{1\linewidth}{!}{
    \begin{tikzpicture} \begin{axis}[
  xmin=-1, xmax=101,
  ymin=-1, ymax=101,
]
\addplot+[
  only marks,
  mark = square*,
  fill=blue,
  color=blue,
  mark size=2.9pt
  ]
  coordinates{
  (90,10)
  (10,90)};
  \end{axis}
  \end{tikzpicture}
}
\end{subfigure}  
\hfill
\begin{subfigure}[t]{0.19\linewidth}
         \centering
\resizebox{1\linewidth}{!}{
    \begin{tikzpicture} \begin{axis}[
  xmin=-1, xmax=101,
  ymin=-1, ymax=101,
]  \addplot+[
  only marks,
  mark = square*,
  fill=blue,
  color=blue,
  mark size=2.9pt
  ]
  coordinates{
  (80,20)
  (20,80)};
  \end{axis}
  \end{tikzpicture}
}
\end{subfigure}  
\hfill
\begin{subfigure}[t]{0.19\linewidth}
         \centering
\resizebox{1\linewidth}{!}{
    \begin{tikzpicture} \begin{axis}[
  xmin=-1, xmax=101,
  ymin=-1, ymax=101,
]
\addplot+[
  only marks,
  mark = square*,
  fill=blue,
  color=blue,
  mark size=2.9pt
  ]
  coordinates{
  (70,30)
  (30,70)};
  \end{axis}
  \end{tikzpicture}
}
\end{subfigure} 
\hfill
\begin{subfigure}[t]{0.19\linewidth}
         \centering
\resizebox{1\linewidth}{!}{
    \begin{tikzpicture} \begin{axis}[
  xmin=-1, xmax=101,
  ymin=-1, ymax=101,
]
\addplot+[
  only marks,
  mark = square*,
  fill=blue,
  color=blue,
  mark size=2.9pt
  ]
  coordinates{
  (60,40)
  (40,60)};
  \end{axis}
  \end{tikzpicture}
}
\end{subfigure}
    \caption{Budgets for trivial task}
    \label{fig:TrivialBudgets}
\end{figure}






\begin{figure}[htbp]
    \centering
\begin{subfigure}[t]{0.19\linewidth}
         \centering
\resizebox{1\linewidth}{!}{
    \begin{tikzpicture} \begin{axis}[
  xmin=-1, xmax=101,
  ymin=-1, ymax=101,
]  \addplot+[
  only marks,
  mark = square*,
  fill=blue,
  color=blue,
  mark size=2.9pt
  ]
  coordinates{ 
  (68, 16)
  (40, 30)
  (88, 6)
  (34, 33)};
\addplot+[
  only marks,
  mark = square*,
  color=red,
  fill=red,
  mark size=2.9pt
  ]
  coordinates{
  (55, 15)
  (20, 40)
};
  \end{axis}
  \end{tikzpicture}
}
\end{subfigure}   
\hfill
\begin{subfigure}[t]{0.19\linewidth}
         \centering
\resizebox{1\linewidth}{!}{
    \begin{tikzpicture} \begin{axis}[
  xmin=-1, xmax=101,
  ymin=-1, ymax=101,
]
\addplot+[
  only marks,
  mark = square*,
  fill=blue,
  color=blue,
  mark size=2.9pt
  ]
  coordinates{
  (40, 20)
  (91, 3)
  (34, 22)
  (70, 10)
  };
\addplot+[
  only marks,
  mark = square*,
  color=red,
  fill=red,
  mark size=2.9pt
  ]
  coordinates{
  (50, 10)
  (13, 27)
};
  \end{axis}
  \end{tikzpicture}
}
\end{subfigure}  
\hfill
\begin{subfigure}[t]{0.19\linewidth}
         \centering
\resizebox{1\linewidth}{!}{
    \begin{tikzpicture} \begin{axis}[
  xmin=-1, xmax=101,
  ymin=-1, ymax=101,
]  \addplot+[
  only marks,
  mark = square*,
  fill=blue,
  color=blue,
  mark size=2.9pt
  ]
  coordinates{
  (10, 70)  
  (20, 40)
  (22, 34)
  (3, 91)};
\addplot+[
  only marks,
  mark = square*,
  color=red,
  fill=red,
  mark size=2.9pt
  ]
  coordinates{
  (10, 50)
  (27, 13)
};
  \end{axis}
  \end{tikzpicture}
}
\end{subfigure}  
\hfill
\begin{subfigure}[t]{0.19\linewidth}
         \centering
\resizebox{1\linewidth}{!}{
    \begin{tikzpicture} \begin{axis}[
  xmin=-1, xmax=101,
  ymin=-1, ymax=101,
]
\addplot+[
  only marks,
  mark = square*,
  fill=blue,
  color=blue,
  mark size=2.9pt
  ]
  coordinates{
  (100, 0)
  (50, 10)
  (20, 16)
  (30, 14)
};
\addplot+[
  only marks,
  mark = square*,
  color=red,
  fill=red,
  mark size=2.9pt
  ]
  coordinates{
  (60, 4)
  (10, 18)
};
  \end{axis}
  \end{tikzpicture}
}
\end{subfigure} 
\hfill
\begin{subfigure}[t]{0.19\linewidth}
         \centering
\resizebox{1\linewidth}{!}{
    \begin{tikzpicture} \begin{axis}[
  xmin=-1, xmax=101,
  ymin=-1, ymax=101,
]
\addplot+[
  only marks,
  mark = square*,
  fill=blue,
  color=blue,
  mark size=2.9pt
  ]
  coordinates{
  (16, 20)
  (0, 100)
  (10, 50)
  (14, 30)
  };
\addplot+[
  only marks,
  mark = square*,
  color=red,
  fill=red,
  mark size=2.9pt
  ]
  coordinates{
  (4, 60)
  (18, 10)
};
  \end{axis}
  \end{tikzpicture}
}
\end{subfigure}
    \caption{Budgets for simple task}
    \label{fig:SimpleBudgets}
\end{figure}









\begin{figure}[htbp]
    \centering
\begin{subfigure}[t]{0.19\linewidth}
         \centering
\resizebox{1\linewidth}{!}{
    \begin{tikzpicture} \begin{axis}[
  xmin=-1, xmax=101,
  ymin=-1, ymax=101,
]  \addplot+[
  only marks,
  mark = square*,
  fill=blue,
  color=blue,
  mark size=2.9pt
  ]
  coordinates{
  (68, 16)
  (40, 30)
  (88, 6)
  (34, 33)};

\addplot+[
%  only marks,
%  mark = square*,
  fill=blue!60,
  color=blue,
  fill opacity=0.1
%  mark size=2.9pt
  ]
  coordinates{
  (0,0)
  (88,0)
  (88, 6)
  (68, 16)
%  (55, 15)
  (40, 30)
  (34, 33)
  (20, 40)
  (0,40)
  };
\addplot+[
  only marks,
  mark = square*,
  color=red,
  fill=red,
  mark size=2.9pt
  ]
  coordinates{
  (55, 15)
  (20, 40)
};
  \end{axis}
  \end{tikzpicture}
}
\end{subfigure}   
\hfill
\begin{subfigure}[t]{0.19\linewidth}
         \centering
\resizebox{1\linewidth}{!}{
    \begin{tikzpicture} \begin{axis}[
  xmin=-1, xmax=101,
  ymin=-1, ymax=101,
]
\addplot+[
  only marks,
  mark = square*,
  fill=blue,
  color=blue,
  mark size=2.9pt
  ]
  coordinates{
  (40, 20)
  (91, 3)
  (34, 22)
  (70, 10)
};

\addplot+[
%  only marks,
%  mark = square*,
  fill=blue!60,
  color=blue,
  fill opacity=0.1
%  mark size=2.9pt
  ]
  coordinates{
  (0,0)
  (91,0)
  (91, 3)
  (70, 10)
  (40, 20)
  (34, 22)
  (13, 27)
  (0,27)
  (0,0)
%  (50, 10)
  };
\addplot+[
  only marks,
  mark = square*,
  color=red,
  fill=red,
  mark size=3pt
  ]
  coordinates{
  (50, 10)
  (13, 27)
};
  \end{axis}
  \end{tikzpicture}
}
\end{subfigure}  
\hfill
\begin{subfigure}[t]{0.19\linewidth}
         \centering
\resizebox{1\linewidth}{!}{
    \begin{tikzpicture} \begin{axis}[
  xmin=-1, xmax=101,
  ymin=-1, ymax=101,
]  \addplot+[
  only marks,
  mark = square*,
  fill=blue,
  color=blue,
  mark size=2.9pt
  ]
  coordinates{
  (10, 70)
  (20, 40)
  (22, 34)
  (3, 91)};
\addplot+[
%  only marks,
%  mark = square*,
  fill=blue!60,
  color=blue,
  fill opacity=0.1
%  mark size=2.9pt
  ]
  coordinates{
  (0,0)
  (0,91)
  (3, 91)
  (10, 70)
%  (10, 50)
  (20, 40)
  (22, 34)
  (27, 13)
  (27,0)
  (0,0)
  };
\addplot+[
  only marks,
  mark = square*,
  color=red,
  fill=red,
  mark size=2.9pt
  ]
  coordinates{
  (10, 50)
  (27, 13)
};
  \end{axis}
  \end{tikzpicture}
}
\end{subfigure}  
\hfill
\begin{subfigure}[t]{0.19\linewidth}
         \centering
\resizebox{1\linewidth}{!}{
    \begin{tikzpicture} \begin{axis}[
  xmin=-1, xmax=101,
  ymin=-1, ymax=101,
]
\addplot+[
  only marks,
  mark = square*,
  fill=blue,
  color=blue,
  mark size=2.9pt
  ]
  coordinates{
  (100, 0)
  (50, 10)
  (20, 16)
  (30, 14)
};
\addplot+[
%  only marks,
%  mark = square*,
  fill=blue!60,
  color=blue,
  fill opacity=0.1
%  mark size=2.9pt
  ]
  coordinates{
  (100, 0)
  (50, 10)
  (20, 16)
  (30, 14)
%  (60, 4)
  (10, 18)
  (0,18)
  (0,0)
  (100,0)
  };
\addplot+[
  only marks,
  mark = square*,
  color=red,
  fill=red,
  mark size=2.9pt
  ]
  coordinates{
  (60, 4)
  (10, 18)
};
  \end{axis}
  \end{tikzpicture}
}
\end{subfigure} 
\hfill
\begin{subfigure}[t]{0.19\linewidth}
         \centering
\resizebox{1\linewidth}{!}{
    \begin{tikzpicture} \begin{axis}[
  xmin=-1, xmax=101,
  ymin=-1, ymax=101,
]
\addplot+[
  only marks,
  mark = square*,
  fill=blue,
  color=blue,
  mark size=2.9pt
  ]
  coordinates{
  (16, 20)
  (0, 100)
  (10, 50)
  (14, 30)
  
  };
\addplot+[
%  only marks,
%  mark = square*,
  fill=blue!60,
  color=blue,
  fill opacity=0.1
%  mark size=2.9pt
  ]
  coordinates{
  (0, 100)
  (10, 50)
  (18, 10)
  (16, 20)
  (14, 30)
%  (4, 60)
  (18,0)
  (0,0)
  (0,100)
  };
\addplot+[
  only marks,
  mark = square*,
  color=red,
  fill=red,
  mark size=2.9pt
  ]
  coordinates{
  (4, 60)
  (18, 10)
};
  \end{axis}
  \end{tikzpicture}
}
\end{subfigure}
    \caption{Budgets for complex task}
    \label{fig:ComplexBudgets}
\end{figure}
